Counter Turing Test ($CT^2$): Investigating AI-Generated Text Detection for Hindi -- Ranking LLMs based on Hindi AI Detectability Index ($ADI_{hi}$)

The widespread adoption of Large Language Models (LLMs) and awareness around multilingual LLMs have raised concerns regarding the potential risks and repercussions linked to the misapplication of AI-generated text, necessitating increased vigilance. While these models are primarily trained for English, their extensive training on vast datasets covering almost the entire web, equips them with capabilities to perform well in numerous other languages. AI-Generated Text Detection (AGTD) has emerged as a topic that has already received immediate attention in research, with some initial methods having been proposed, soon followed by the emergence of techniques to bypass detection. In this paper, we report our investigation on AGTD for an indic language Hindi. Our major contributions are in four folds: i) examined 26 LLMs to evaluate their proficiency in generating Hindi text, ii) introducing the AI-generated news article in Hindi ($AG_{hi}$) dataset, iii) evaluated the effectiveness of five recently proposed AGTD techniques: ConDA, J-Guard, RADAR, RAIDAR and Intrinsic Dimension Estimation for detecting AI-generated Hindi text, iv) proposed Hindi AI Detectability Index ($ADI_{hi}$) which shows a spectrum to understand the evolving landscape of eloquence of AI-generated text in Hindi. The code and dataset is available at https://github.com/ishank31/Counter_Turing_Test

==> 5_watermarking.tex <==
\section{Watermarking}

==> Hindi_examples.tex <==


\begin{table}[]
\begin{tabular}{@{}c|l@{}}
\toprule
\textbf{Field} & \multicolumn{1}{c}{\textbf{Content}} \\ \midrule
Headline & \texthindi{पीएम मोदी के ग्रीस दौरे के बाद अदानी के नाम की चर्चा क्यों?} \\ \midrule
\begin{tabular}[c]{@{}c@{}}Human-written\\ article\end{tabular} & \begin{tabular}[c]{@{}l@{}} \texthindi{कांग्रेस पार्टी ने एक बार फिर पीएम मोदी पर अदानी समूह को फ़ायदा पहुँचाने के लिए विदेश यात्रा पर जाने}\\ \texthindi{का आरोप लगाया है. बीजेपी के प्रवक्ता ने इन आरोपों को बेबुनियाद बताया है जबकि अदानी समूह ने इसे} \\ \texthindi{कयासबाज़ी बताया है. पीएम मोदी पिछले हफ़्ते ग्रीस दौरे पर गए थे. पिछले 40 सालों में किसी भारतीय} \\ \texthindi{प्रधानमंत्री का ये पहला दौरा था. इससे पहले साल 1983 में भारत की तत्कालीन प्रधानमंत्री इंदिरा गांधी} \\ \texthindi{ग्रीस पहुंची थीं जो भूमध्य सागर क्षेत्र में भारत के लिए रणनीतिक रूप से काफ़ी अहम है. पीएम मोदी ने ग्रीस}\\ \texthindi{पहुँचकर कहा था, "चालीस सालों बाद भारत के किसी प्रधानमंत्री का ग्रीस आना हुआ है. फिर भी, ना तो} \\ \texthindi{हमारे संबंधों की गहराई कम हुई है, ना ही रिश्तों की गर्मजोशी में कोई कमी आई है." इंदिरा गांधी 23 सितंबर} \\ \texthindi{को ग्रीस में स्थानीय नेताओं के साथ लेकिन इसके बाद भी पीएम मोदी ने ग्रीस में सिर्फ़ कुछ घंटे ही गुज़ारे.} \\ \texthindi{पीएम मोदी दक्षिण अफ़्रीका में आयोजित हुए ब्रिक्स सम्मेलन से लौटते हुए ग्रीस पहुंचे थे. और इसके तुरंत} \\ \texthindi{बाद उन्हें बेंगलुरू पहुंचकर इसरो के वैज्ञानिकों से मुलाक़ात करनी थी. लेकिन इतने संक्षिप्त दौरे और व्यस्त} \\ \texthindi{कार्यक्रम के बावजूद भारत में काम कर रही कई कंपनियों के शीर्ष अधिकारी ग्रीस पहुंचकर पीएम मोदी के} \\ \texthindi{साथ उस बिज़नेस लंच में शामिल हुए जिसे ग्रीक पीएम ने आयोजित किया था.इस मौके पर ग्रीस के} \\ \texthindi{व्यापारिक जगत के शीर्ष अधिकारियों ने भारतीय व्यापारिक हस्तियों से मुलाक़ात की.}\end{tabular} \\ \midrule
GPT-4 & \begin{tabular}[c]{@{}l@{}}\texthindi{प्रधानमंत्री नरेंद्र मोदी के हालिया ग्रीस दौरे के बाद व्यापारिक जगत में अदानी समूह के नाम की खूब चर्चाएँ} \\ \texthindi{हो रही हैं। इस दौरे का मुख्य आकर्षण था द्विपक्षीय संबंधों की मजबूती और व्यापारिक सहयोग के नए} \\ \texthindi{आयामों का विस्तार। ग्रीस के साथ भारत के संबंध पारंपरिक रूप से मजबूत रहे हैं, और इस दौरे के द्वारा} \\ \texthindi{उन्होंने नई ऊर्जा का संचार किया। प्रधानमंत्री मोदी ने ग्रीस के राजनीतिक नेतृत्व और व्यापारिक प्रतिनिधियों} \\ \texthindi{के साथ गहन वार्ता की, जिसमें कई रणनीतिक साझेदारियां और समझौते सामने आए। लेकिन इन सबके बीच} \\ \texthindi{जो मुख्य मुद्दा उभर कर आया, वह था अदानी समूह की व्यापारिक विस्तार योजनाएँ। अदानी समूह, जो कि} \\ \texthindi{भारत के प्रमुख उद्योगपतियों में से एक है, वह ग्लोबल इंफ्रास्ट्रक्चर, लॉजिस्टिक्स, ऊर्जा सेक्टर में अपनी} \\ \texthindi{पहुंच बढ़ाने की तलाश में है। इस दौरे के दौरान, ग्रीस के साथ हुए समझौतों में अदानी समूह को कुछ महत्वपूर्ण}\\ \texthindi{परियोजनाओं के लिए विचार-विमर्श के अवसर प्राप्त हुए। जानकारी के अनुसार, अदानी समूह ग्रीस में नवीन} \\ \texthindi{ऊर्जा, पोर्ट डेवलपमेंट और अन्य बुनियादी ढांचे की परियोजनाओं में निवेश करने का इच्छुक है}\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}c|l@{}}
\toprule
\textbf{Field} & \multicolumn{1}{c}{\textbf{Content}} \\ \midrule
Headline & \texthindi{पीएम मोदी के ग्रीस दौरे के बाद अदानी के नाम की चर्चा क्यों?} \\ \midrule
GPT-3.5 & \begin{tabular}[c]{@{}l@{}}\texthindi{प्रधानमंत्री नरेंद्र मोदी के सम्राटी ग्रीस दौरे सफलतापूर्वक समाप्त हो चुके हैं। इस दौरे ने उपनगरीयों के दिलों में}  \\ \texthindi{एक तरंग उठाई है जिसके कारण देश भर में यह सवाल उठ रहा है कि पीएम मोदी के इस ग्रीस दौरे के बाद क्यों} \\  \texthindi{अदानी के नाम की चर्चा हो रही है। भारतीय व्यापारी और उद्योगपति मुकेश अनिल अम्बानी, जिन्हें देशभर में} \\ \texthindi{व्यापार का सर्वश्रेष्ठ ध्येय बताया जाता है, अपनी बदौलत एक आदर्श नागरिक के रूप में मान्यता प्राप्त कर चुके} \\ \texthindi{हैं। उनकी सफलता की कहानियाँ बच्चों और युवाओं के बीच मोटिवेशनल कहानियों के रूप में फैल चुकी हैं। इन}\\ \texthindi{नागरिकों के लिए, प्रधानमंत्री मोदी और मुकेश अम्बानी के नाम समानरूप से जुड़े हुए हैं। इस ध्यासी और सतत} \\ \texthindi{कामकाज के बीच पीएम मोदी ने हाल ही में एक अत्याधुनिक और नवीनतम ग्रीस यात्रा की है, जिसने लोगों के} \\ \texthindi{आंदोलन साधारित हो दिए हैं। इस यात्रा के कारण, अखबारों, मीडिया में एक नई परिचर्चा पर चर्चा हो रही है।}\\ \texthindi{पीएम मोदी के इस ग्रीस दौरे से होते हुए उनके बड़े और प्रमुख समर्थक, मुकेश अम्बानी का नाम जुड़ा हुआ आया} \\ \texthindi{है। विपक्षी दलों ने प्रमुख व्यापारी और उद्योगपति मुकेश अम्बानी के नाम से योग्यानुयोग प्रस्ताव रखने का आरोप} \\ \texthindi{लगाया है। वे दावा करते हैं कि प्रधानमंत्री ने यात्रा के दौरान अदानी के साथ व्‍यापारिक उद्योगों को बढ़ावा दिया है।} \\ \texthindi{इसके अलावा, अदानी के कुछ सौभाग्यशाली व्‍यापारिक उद्योगों के मध्य कई समझौतों की खबरें भी आ रही हैं।} \\\texthindi{ प्रधानमंत्री नरेंद्र मोदी ने इस आरोप का कड़ी निंदा करते हुए कहा है कि ये एक गलत आरोप है और जो भी समझौते}\\ \texthindi{हुए हैं, वे अमनचंद्र अदानी तथा उनके व्यापारिक उघारों के खातिर हुए हैं, बिना किसी राजनीतिक दबाव के। इन} \\ \texthindi{सारे कार्यक्रमों, समारोहों और सम्मेलनों के बावजूद, प्रधानमंत्री विदेश में जाते ही पर्यटन, वाणिज्य, उभरने वाली} \\ \texthindi{शिक्षा, वित्तीय खातों का मामला, उद्योग जगत को मिल रहे लाभ, बेरोजगारी दूर करने के बारे में सवाल उठाया गया} \\ \texthindi{है। अदानी के नाम की चर्चा होने से पता चलता है कि नागरिक समाज में कई राजनीतिक और आर्थिक मुद्दों पर चर्चा} \\ \texthindi{हो रही है। प्रधानमंत्री मोदी के ग्रीस दौरे की सफलता और अदानी के नाम से जुड़े तर्कों को ध्यान में रखते हुए, देशभर} \\ \texthindi{में यह भी मान्यता प्राप्त हो रहा है कि अदानी भारतीय उद्योग में एक बड़ी किंवदंती हैं। इसलिए, प्रधानमंत्री के नाम से} \\ \texthindi{जुड़े ग्रीस दौरे के बाद अदानी के नाम की चर्चा स्वाभाविक रूप से बढ़ी है। संक्षेप में कहें तो, पीएम मोदी के ग्रीस यात्रा} \\ \texthindi{के बाद क्यों अदानी के नाम की चर्चा हो रही है, इसका मुख्य कारण उनके द्वारा संचालित व्यापारिक उद्योगों में भारी} \\ \texthindi{सफलता होने से है। इसके अलावा, प्रधानमंत्री और उद्योगपति मुकेश अम्बानी के बीच के गहरे रिश्ते ने इस चर्चा को} \\ \texthindi{और भी तेजी से बढ़ाया है।}\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}c|l@{}}
\toprule
\textbf{Field} & \multicolumn{1}{c}{\textbf{Content}} \\ \midrule
Headline & \texthindi{पीएम मोदी के ग्रीस दौरे के बाद अदानी के नाम की चर्चा क्यों?} \\ \midrule
BARD & \begin{tabular}[c]{@{}l@{}}\texthindi{भारत के प्रधानमंत्री नरेंद्र मोदी ने 20 जुलाई, 2023 को ग्रीस की यात्रा की। इस यात्रा के दौरान, उन्होंने ग्रीस} \\ \texthindi{के राष्ट्रपति काकलिस और प्रधानमंत्री मित्सोटाकिस से मुलाकात की। इन मुलाकातों के दौरान, दोनों देशों ने} \\ \texthindi{कई क्षेत्रों में सहयोग बढ़ाने पर सहमति व्यक्त की।इन सहमतियों में से एक अदानी समूह की ग्रीस में निवेश करने} \\ \texthindi{की संभावना पर चर्चा शामिल थी। अदानी समूह एक भारतीय बहुराष्ट्रीय समूह है जो बुनियादी ढांचा, ऊर्जा,} \\ \texthindi{परिवहन, और अन्य क्षेत्रों में काम करता है। अदानी समूह के ग्रीसमें निवेश करने की संभावना पर चर्चा होने के} \\ \texthindi{बाद, अदानी के नाम की चर्चा फिर से शुरू हो गई। यह चर्चा कई कारणों से हो रही है। एक कारण यह है कि} \\ \texthindi{अदानी समूह भारतका सबसे बड़ा निजी निवेशक है। समूह की कुल संपत्ति लगभग 150 अरब डॉलर है। अदानी} \\ \texthindi{समूह ने पिछले कुछ वर्षों में भारत में कई बड़ी परियोजनाओं में निवेश किया है,जिसमें बंदरगाह, हवाई अड्डे, और} \\ \texthindi{बिजली स्टेशन शामिल हैं। दूसरा कारण यह है कि अदानी समूह पर कुछ विवादों का सामना करना पड़ रहा है।} \\ \texthindi{इन विवादों में अदानी समूह के परियोजनाओं के लिए सरकार से अनुचित लाभ प्राप्त करने के आरोप शामिल हैं।} \\ \texthindi{पीएम मोदी के ग्रीस दौरे के बाद अदानी के नाम की चर्चा के कुछ संभावित कारण इस प्रकार हैं:} \\ \texthindi{अदानी समूह के ग्रीस में निवेश करने की संभावना पर चर्चा होने से, अदानी समूह को भारत के बाहर एक बड़ी} \\ \texthindi{भूमिका निभाने के अवसर मिल सकते हैं। अदानी समूह पर विवादों के बीच, अदानी के नाम की चर्चा से विवादों}  \\ \texthindi{को और बढ़ाने का खतरा है। अदानी समूह के ग्रीस में निवेश करने की संभावना पर चर्चा होने से, भारत और ग्रीस} \\ \texthindi{के बीच संबंधों को मजबूत करने में मदद मिल सकती है। अदानी समूह के ग्रीस में निवेश करने की संभावना का} \\ \texthindi{भारत और ग्रीस दोनों देशों के लिए महत्वपूर्ण आर्थिक और राजनीतिक निहितार्थ हो सकते हैं।} \end{tabular} \\ \midrule
Gemma-2B & \begin{tabular}[c]{@{}l@{}}\texthindi{पीएम मोदी के ग्रीस दौरे के बाद अदानी के नाम की चर्चा क्यों?} \\ \texthindi{देश में पीएम मोदी के ग्रीस दौरे के बाद अदानी नाम की चर्चा में कमी आ रही है। इस दौरे में, अदानी को भारत}  \\ \texthindi{में ग्रीस के खिलाड़ी के रूप में मानने का आरोप लगाया गया है। इस दौरे के बाद अदानी के नाम को कई लोगों}  \\ \texthindi{में आकर्षित किया है। हमें से कुछ लोग अदानी को एक स्वच्छ और शिक्षित व्यक्ति के रूप में मानते हैं, जबकि} \\ \texthindi{अन्य लोग अदानी को एक अविताम और शक्त व्यक्ति के रूप में मानते हैं। इस दौरे के बाद अदानी के नाम को} \\ \texthindi{आकर्षित करने में सहायक में शामिल हैं: अदानी का पारस्परिक संबंध पीएम मोदी से, अदानी का शिक्षा और} \\ \texthindi{अनुभव, अदानी का मान्यता और विश्वास, अदानी का आत्मविश्वास और स्वच्छता इस दौरे के बाद अदानी को} \\ \texthindi{भारत में ग्रीस के खिलाड़ी के रूप में मानने का आरोप लगाया गया है। हमें से कुछ लोग अदानी को एक स्वच्छ} \\ \texthindi{और शिक्षित व्यक्ति के रूपमें मानते हैं, जबकि अन्य लोग अदानी को एक अविताम और शक्त व्यक्ति के रूप में} \\ \texthindi{मानते हैं।} \end{tabular} \\ \midrule
Gemma-7B & \begin{tabular}[c]{@{}l@{}}\texthindi{पीएम मोदी के ग्रीस दौरे के बाद अदानी के नाम की चर्चा क्यों?} \\ \texthindi{अनकंडा, 10 नवंबर - प्रधानमिन मोदी के ग्रीस दौरे के बाद अदानी समूह के नाम की चर्चा शुरू हुई है। दौरे के} \\ \texthindi{दौरान, मोदी और ग्रीस के प्रधानमिन के बीच अदानी समूह के लिए एक समझौदा हुआ था। दौरे के बाद, अदानी} \\ \texthindi{समूह के शेयरों में उछौल देख गया है। कुछ विशेषजों का मानना है कि अदानी समूह के लिए ग्रीस दौरे के बाद के} \\ \texthindi{अवसरों में सुधार लाए हैं। अदानी समूह के लिए ग्रीस दौरे के बाद के अवसरों में सुधार लाए हैं। प्रधानमिन मोदी के} \\ \texthindi{ग्रीस दौरे के बाद अदानी के नाम की चर्चा के कुछ कारण हैं: अदानी और ग्रीस के बीच समझौदा: दौरे के दौरान,} \\ \texthindi{मोदी और ग्रीस के प्रधानमिन के बीच अदानी समूह के लिए एक समझौदा हुआ था। समझौदा के अनुसार, अदानी}  \\ \texthindi{समूह ग्रीस में एक बड़े प्रौद्योगिकी के लिए संयंत्र स्थापित करेगा। अदानी के शेयरों में उछौल: दौरे के बाद, अदानी} \\ \texthindi{समूह के शेयरों में उछौल देख गया है। विशेषजों का मानना: कुछ विशेषजों का मानना है कि अदानी समूह के लिए} \\ \texthindi{ग्रीस दौरे के बाद के अवसरों में सुधार लाए हैं। अदानी समूह के लिए ग्रीस दौरे के बाद के अवसरों में सुधार लाए हैं।} \end{tabular} \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[]
\begin{tabular}{@{}cl@{}}
\toprule
\textbf{Field} & \multicolumn{1}{c}{\textbf{Content}} \\ \midrule
\multicolumn{1}{c|}{Headline} & \texthindi{मधुमिता शुक्ला हत्याकांड: अमरमणि त्रिपाठी और उनकी पत्नी के जेल जाने की कहानी.} \\ \midrule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Human-written\\ article\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\texthindi{अगस्त 2023 नौ मई, 2003 को लखनऊ के तक़रीबन सभी वरिष्ठ पुलिस अधिकारी एक ख़ास} \\ \texthindi{बैठक में व्यस्त थे. शाम के चार बजे से चल रही इस बैठक में अगले दिन यानी 10 मई को शहर} \\ \texthindi{में होने वाले चुप ताज़िया के जुलूस की तैयारियों पर चर्चा हो रही थी. मोहर्रम के दौरान निकलने} \\ \texthindi{वाले हज़ारों लोगों के इस जुलूस की सुरक्षा व्यवस्था लखनऊ पुलिस के लिए हमेशा से चुनौती} \\ \texthindi{रही थी.}\end{tabular} \\ \midrule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}GPT-2\\ (English output)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}May 15, 2017 The article was written by a journalist who was not a journalist.\\ The article was published on May 15 and was published in the Hindustan Times.\\ In the article, the journalist said that the BJP government has been trying to get \\ the Congress to give the Congress a platform to run the country. \\ @jamesharan\_nagar @jameshaan\_nao\end{tabular} \\ \midrule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}GPT-2 XL\\ (Code-switching)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\texthindi{मधुमिता शुक्ला हत्याकांड: अमरमणि त्रिपाठी और उनकी पत्नी के जेल जाने की कहानीं का क क}\\ \texthindi{। क  सर्।ि।ी।}\textbackslash{}n\textbackslash{}nThe article is written in Hindi and the headline is written as \\ मु मारात शाही: स् म म १५॥ In the above example, the Hindi word म is used to \\ indicate the noun म. The word श is used for the adjective शि. The adjective साम is\\ also used for स. The noun क is used in the article to indicate a noun.\end{tabular} \\ \midrule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Mistral-7B\\ instruct\\ (Gibberish output)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\texthindi{मधुमिता शुक्ला हत्याकांड: अमरमणि त्रिपाठी और उनकी पत्नी के जेल जाने की कहानी मधुमाता} \\ \texthindi{शुक्ला हत्याकांड वालों की उनको जेल जाने की कहानी है। उनकें नहीं उनको शुचिती हमारी पुरानों} \\ \texthindi{की संस्करण पहले अवश्यक होता है। उनको जेल जाने की कहानी बहुती है। आजकल समस्यों को} \\ \texthindi{अलग उनको जेल जाने को अलग नहीं किया जाता है।} \end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

==> Results.tex <==

%\subsection{Evaluation}

%This section discusses the results based on the models discussed in the previous section. 
%The results can be reproduced using the code and data available here \footnote{\url{http://bit.ly/3Ts0BwJ}} .

\noindent
\textbf{RADAR:}
Results from Table \ref{tab:Main_results} showcases RADAR's sub-par performance across models. We observe that the accuracy of detecting GPT4 and GPT3.5 responses fall below 50\%, indicating a performance lower than that of a random classifier. RADAR fails to detect any GPT3.5 responses as AI-generated resulting in an F1-score of 0. This score stands the lowest among all the models assessed. Although responses from BARD and Gemma-7B demonstrate higher level of detectability compared to other models, they still exhibit an sub-optimal overall performance  . Notably, higher precision values compared to recall values across models suggest that while the model is able to classify human-written text as such, it fails to identify the AI-generated text. Consistent low accuracy and F1-scores across models show that RADAR struggles in detecting AI-generated text accurately.


\noindent
\textbf{Intrinsic Dimension estimation:}
In line with the methodology employed by \cite{tulchinskii2023intrinsic}, we present the Maximum Likelihood estimation (MLE) along with the PHD estimations. \cite{tulchinskii2023intrinsic} show that the PHD of most European languages is approximately \textbf{9$\pm$1}. However, our experiments reveal that the PHD of Hindi language is lower and lies in the range of \textbf{6 to 7}. Moreover, the MLE values lie in the range of \textbf{9 to 10}. As shown in Table \ref{tab:Main_results}, different models exhibit distinct PHD and MLE values. The responses from GPT-4, GPT-3.5 and BARD exhibit intrinsic dimensions similar to those of human texts, posing a challenge in distinguishing  these responses as AI-generated. Consequently, the disparity in the intrinsic dimensions of the Gemma models and human texts makes their responses more readily discernible as AI-generated. Fig \ref{fig:IntrinsicDim-MLE} and Fig \ref{fig:IntrinsicDim-PHD} show the comparison of distribution of the values across models.



\noindent
\textbf{J-Guard:}
J-Guard showcases superior performance in detecting AI-generated text as such. We observe that the J-Guard framework shows significantly higher performance than the other methods discussed. High F1-scores across models indicate J-Guard's efficiency in accurately differentiating between human and AI-generated text. The model extracts journalistic features such as date and time formats, structural features like mean word count, word count of leading paragraph, word count of leading sentence, mean sentence count, and punctuation usage. Since the model learns for these features and the data consists of news articles, this might explain the model's high performance. The cross-model metrics can be found in Appendix \ref{sec:J-guard}.
 
\vspace{1mm}

\noindent
\textbf{ConDA:}
ConDA exhibits notably poor performance while classifying human and AI-generated text. Low accuracy, precision, recall and F1-score falling below 50\% indicate that ConDA struggles significantly in the task. An accuracy of less than 50\% indicates that the model's performance is worse than that of a random guesser. Low precision and recall scores indicate that the model frequently misclassifies AI-generated text as human-written and vice a versa. These scores result in a low F1-score. 


\noindent
\textbf{RAIDAR:}
RAIDAR analyzes the alterations made by the LLM while rewriting a given text to disntinguish between human and AI-generated text. We experiment with six prompts to rewrite the samples from the dataset. More information about the prompts used can be found in Appendix \ref{sec:RAIDAR_appendix}. We observe that responses of Gemma models is highly detectable, whereas GPT-4, GPT-3.5 and BARD responses are difficult to detect. The stark 30-35\% difference in accuracy and F1-score between GPT models and Gemma models suggest that the GPT models generate more human-like responses. These human-like responses lead to fewer modifications while rewriting the given text, resulting in lower detectability.  

\vspace{-2mm}







==> fig.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{img/AGTD_example_rejected_models.pdf}
    \caption{This figure illustrates the outputs from the models that were rejected. The initial lines of the articles are displayed, with the content in blue text representing a translation for better understanding. As excluded models do not provide accurate Hindi responses, their translations are not presented.}
    \label{fig:rejected_output}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{img/AGTD_example_best_worst_model.pdf}
    \caption{This figure represents the outputs from LLMs for generating Hindi news articles using BEST and WORST model respectively. The initial lines of the articles are displayed, with the content in blue text representing a translation for better understanding.}
    \label{fig:example}
\end{figure*}

\begin{tcolorbox}
[colback=blue!5!white,colframe=blue!65!black,title=\textbf{\footnotesize \textsc{Our Contributions}:} {\footnotesize A Counter Turing Test (\textbf{CT}$^2$) and AI Detectability Index (ADI) for Hindi.}]

\vspace{-2mm}
\begin{itemize}[leftmargin=1mm]
\setlength\itemsep{0em}
\begin{spacing}{0.85}
    \item[\ding{224}]{\footnotesize 
    {\fontfamily{phv}\fontsize{8}{9}\selectfont
    Introducing the \emph{\ul{Hindi Counter Turing Test (CT$^2$)}}, a benchmark that incorporates methods designed to provide a thorough assessment of the resilience of existing AGTD techniques in Hindi.
    }
    }

    \item[\ding{224}] {\footnotesize 
    {\fontfamily{phv}\fontsize{8}{9}\selectfont
    Demonstrating through empirical evidence that widely used AGTD methods exhibit fragility and are relatively susceptible to evasion.
    }
    
    \item[\ding{224}] {\fontfamily{phv}\fontsize{8}{9}\selectfont
    Presenting the \textit{\ul{AI Detectability Index for Hindi ($ADI_{hi}$)}} as a metric for Language Models to assess whether their outputs can be identified as generated by artificial intelligence or not.} 
    }
    
    \item[\ding{224}] {\footnotesize 
    {\fontfamily{phv}\fontsize{8}{9}\selectfont
    Conducting a thorough examination of 16 contemporary LLMs to generate dataset}
    }
    
    \item[\ding{224}] {\footnotesize 
    {\fontfamily{phv}\fontsize{8}{9}\selectfont
    Both benchmarks -- CT$^2$ and $ADI_{hi}$ -- will be published as open-source leaderboards.}
    }
    
    \item[\ding{224}] {\footnotesize 
    {\fontfamily{phv}\fontsize{8}{9}\selectfont 
    Curated datasets will be made available with the MIT License, making it favorable for open-source research and commercial use.
    
    }% for research purposes. 
    }
\vspace{-5mm}
    
\end{spacing}
\end{itemize}
\end{tcolorbox}
